Hull and Geodetic Numbers for Some Classes of Oriented Graphs

Let $D$ be an orientation of a simple graph. Given $u,v\in V(D)$, a directed shortest $(u,v)$-path is a $(u,v)$-geodesic. $S \subseteq V(D)$ is convex if, for every $u,v \in S$, the vertices in each $(u,v)$-geodesic and in each $(v,u)$-geodesic are in $S$. For each $S \subseteq V(D)$ the (convex) hull of $S$, denoted by $[S]$, is the smallest convex set containing $S$. $S \subseteq V(D)$ is a hull set if $[S] = V(D)$. $S \subseteq V(D)$ is a geodetic set of $D$ if each vertex of $D$ lies in a $(u,v)$-geodesic, for some $u,v \in S$. The cardinality of a minimum hull set (resp. geodetic set) of $G$ is the hull number (resp. geodetic number) of $D$, denoted by $ \overrightarrow{\textrm{hn}} (D)$ (resp. $\overrightarrow{\textrm{gn}}(D)$). We first show a tight upper bound on $\overrightarrow{\textrm{hn}}(D)$. Given $k\in\mathbb{Z}_+^*$, we prove that deciding if $\overrightarrow{\textrm{hn}}\leq k$ is NP-complete when $D$ is an oriented partial cube; and if $\overrightarrow{\textrm{gn}}(D)\leq k$ is W[2]-hard parameterized by $k$ and has no $(c \cdot \ln n)$-approximation algorithm, unless P = NP, even if $D$ has an underlying graph that is bipartite or split or cobipartite. We also show polynomial-time algorithms to compute $\overrightarrow{\textrm{hn}}(D)$ and $\overrightarrow{\textrm{gn}}(D)$ when $D$ is an oriented cactus.

==> sec3-boundsplit.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Upper bound on the hull number of an oriented split graph}
\label{section.st}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A graph \( G \) is called a split graph when \( V(G) \) can be partitioned into a clique \( C \) and a stable set \( S \).
Also we often denote a split graph \( G \) as \( G = (S \cup C,E) \).
The hull number problem for (undirected) split graphs has already been studied in~ \cite{OTCOTHNOAG}.
Given a split graph $G=(S \cup C,E)$ with $S$ a maximal stable set and $C$ a clique, the authors prove that $\hn (G) \in \{ |S|,|S|+1,|\ext (G)| \}$. 
Moreover, they prove that $\hn(G)$ can be computed in linear time, when $G$ is split.

Notice that in a split graph the vertices of $S$ are simplicial.
Thus, they belong to any hull set in the non-oriented case.
However, in an orientation of $G$, maybe none of these vertices is extreme.
The extreme vertices of $S$ must be in every hull set of $D$ (an orientation of $G$), leaving the non-extreme vertices of $S$ to analyse.

\begin{lem}
    \label{lemma.non-extremeinS}
    If $D=(S \cup C,A)$ is an oriented split graph, then $S \setminus \ext(D) \subseteq I(C)$.
\end{lem}
\begin{proof}
    Given a non-extreme vertex $v \in S$ (notice that \( d_G(v) \geq 2 \)), by definition there must be $u,w \in C$ such that $(u,v),(v,w),(w,u) \in A(D)$, which means that $v \in I( \{ u,w \} )$.
    Using that argument for every non-extreme vertex of \( S \) gives us the proof of the lemma.
\end{proof}

We then focus on the hull number problem for tournaments.
Up to the end of this section, unless we state otherwise, \( D \) will denote a tournament.

%In the previous case, we concerned ourselves with the extreme vertices, in this one they won't be of any help with the other vertices.

Lemma \ref{lemma.extour} points out that extreme vertices in a tournament have little significance when applying the interval function, because every geodesic such that at least one end-vertex is extreme has only one arc.

\begin{lem}\label{lemma.extour}
    Let $D$ be a tournament and $u,v \in V(D)$ two distinct vertices such that $u \in \ext(D)$.
    Then $I( \{ u,v \} ) = \{ u,v \}$.
\end{lem}

\begin{proof}
    First suppose that \( u \) is a source.
    Since \( D \) is a tournament the only \( (u,v) \)-geodesic has exactly one arc: \( (u,v) \).
    Seen as \( u \) is a source there cannot be a \( (v,u) \)-path, which concludes the argument for \( I( \{ u,v \} ) = \{ u,v \} \).
    The case in which \( u \) is a sink is analogous.

    Now let \( u \) be a transitive extreme vertex.
    Without loss of generality we assume that \( (u,v) \in A(D) \), which means that the only \( (u,v) \)-geodesic has just one arc.
    Suppose that there is a \( (v,u) \)-geodesic \( P = (v=v_0,v_1, \ldots ,v_k=u) \), where \( k \geq 2 \).
    If \( (v_{k-2},u) \in A(D) \) we would have a \( (v,u) \)-path shorter than \( P \), contradicting the fact that it is a geodesic; hence \( (u,v_{k-2}) \in A(D) \).
    However, now the arcs \( (v_{k-2},v_{k-1}),(v_{k-1},u),(u,v_{k-2}) \) contradict the transitivity of \( u \).
    Thus, we reach the conclusion that there cannot be a \( (v,u) \)-path, which implies \( I( \{ u,v \} ) = \{ u,v \} \).
\end{proof}

A consequence of this fact is that \( I(S) = I(S \setminus \ext (D)) \cup (S \cap \ext (D)) \) for every \( S \subseteq V(D) \).
Thus, apart from being required in every hull set, the extreme vertices will not exert any influence on \( V(D) \setminus \ext (D) \) when applying the interval function.

\begin{lem}\label{lemma.extour2}
    If \( D \) is a tournament, then \( S \) is a hull set of \( D \) if and only if \( \ext(D) \subseteq S \) and \( [ S \setminus \ext(D) ] = V(D) \setminus \ext(D) \).
\end{lem}

\begin{proof}
    Let \( X = \ext(D) \) to simplify.
    If \( S \subseteq V(D) \) is such that \( X \subseteq S \) and \( [ S \setminus X ] = V(D) \setminus X \) then \( [ S ] \supseteq [ S \setminus X ] \cup X = V(D) \), which implies that \( S \) is a hull set.

    Now assume that \( S \) is a hull set of \( D \).
    It is straightforward that \(  X \subseteq S \).
    By Lemma \ref{lemma.extour}, we have:
    \begin{equation*}
        \begin{split}
            I(S) &= I(X \cup (S \setminus X)) = \bigcup_{u,v \in S} I( \{ u,v \} )\\
            &= \left( \bigcup_{u,v \in X} I( \{ u,v \} ) \right) \cup \left( \bigcup_{\substack{u \in S \setminus X\\v \in X}} I( \{ u,v \} ) \right) \cup \left( \bigcup_{u,v \in S \setminus X} I( \{ u,v \} ) \right)\\
            &= X \cup \left( X \cup (S \setminus X) \right) \cup I( S \setminus X) = X \cup I( S \setminus X).
        \end{split}
    \end{equation*}
    Since \( I(S \setminus X) \) does not contain any extreme vertex, we can iterate the above argument and claim that \( I^n(S) = X \cup I^n(S \setminus X) \), for every \( n \in \mathbb{N} \).
    We thus conclude that \( V(D) = [S] = X \cup [S \setminus X] \therefore V(D) \setminus X = [S \setminus X] \).
\end{proof}

%This means that the extreme vertices of a tournament, besides belonging to all hull set, do not influence in anything when we apply the interval function on a given vertex subset.
%Thus, in order to obtain a hull set $S \subseteq V(D)$, we must have $S \supseteq \ext(D)$ and $V(D) = \ext(D) \cup [S \setminus \ext(D)]$.

Let us then analyse the non-extreme vertices of $D$.
Given a non-extreme vertex $v \in V(D)$ there must be $u,w \in V(D)$ such that $(u,v),(v,w),(w,u) \in A(D)$, which implies that $u,w$ are also non-extreme vertices.
This means that each non-extreme vertex $v$ lies in a directed $C_3 \subseteq D$, and consequently \( v \) is an internal vertex of an $(u,w)$-geodesic.

Thus, for each non-extreme vertex $v$ that does not belong to a minimum hull set $S$ of $D$, at most two other non-extreme vertices must belong to $S$ to ensure that $v \in [S]$.
%Since we want to use what we prove here for the oriented split graph, the hull number might cause trouble due to de geodesics of length greater than two.
%With that in mind we create a couple of new tools based on the interval function and on the hull of a set.
%We define the function \( I_{\small{\overrightarrow{C3}}} \colon \mathcal{P}(V(D)) \rightarrow \mathcal{P}(V(D)) \) as \( I_{\overrightarrow{C3}}[S] := \{ v \in V(D) \mid \textrm{exists } H \cong C_3 \textrm{ such that } V(H) = \{ u,v,w \} \textrm{ and } u,w \in S \} \).
%Much like the hull of a vertex set, when we iterate the above function in \( S \) and reach a natural \( n \) such that \( I_{\overrightarrow{C3}}^n[S] = I_{\overrightarrow{C3}}^{n+1}[S] \) we define \( [S]_{\overrightarrow{C3}} := I_{\overrightarrow{C3}}^n[S] \).
After presenting a few definitions, we will be ready to prove the main result for tournaments.

Since we will only use \( C_3 \)'s in our arguments, assuming \( |S| \geq 2 \), we define \( I_{\overrightarrow{C3}}(S) := \{ v \mid \textrm{ there are } u,w \in S \textrm{ composing a directed } C_3 \textrm{ with } v \} \cup S \) and \( [S]_{\overrightarrow{C3}} \) analogous to \( [S] \) but using \( I_{\overrightarrow{C3}} \) instead of the interval function $I$.

Let $D$ and $D'$ be oriented graphs.
The \textit{lexicographic product} of $D$ by $D'$, denoted by $D \circ D'$, is the oriented graph which satisfies $V(D \circ D') = V(D) \times V(D')$ and $((u_1,v_1),(u_2,v_2)) \in A(D \circ D')$ if, and only if, either $(u_1,u_2) \in A(D)$ or $u_1 = u_2$ and $(v_1,v_2) \in A(D')$.
In other words, for each vertex $v \in V(D)$ we take a copy of $D'$, namely $D'_v$, and if $(u,v) \in A(D)$, then we add the arcs $(u',v')$, for each $u' \in V(D'_u)$ and each $v' \in V(D'_v)$.

A transitive orientation of a simple graph \( G \) is an oriented graph \( D \) obtained from \( G \) such that every vertex is extreme.
In this case, a transitive orientation of a complete graph is a transitive tournament.

\begin{lem}\label{proposition.tour}
    Let $D$ be a tournament.
    Then $\ohn (D) \leq |\ext (D)| + \frac{2}{3}|V(D) \setminus \ext (D)|$ and this bound is tight.
    Moreover, there is a set $S \subseteq V(D)$ such that $|S| \leq \frac{2}{3}(n(D)-|\ext(D|)$ and \( [S]_{\overrightarrow{C3}} = V(D) \setminus \ext(D)\).
\end{lem}

\begin{proof}
    By Lemma \ref{lemma.extour2}, we have that \( S' = \ext(D) \cup S \) with \( \ext(D) \cap S = \emptyset \) is a hull set of \( D \) if and only if \( [ S ] = V(D) \setminus \ext(D) \).
    Thus, we only need to find an \( S \) respecting the conditions as in the statement of the lemma.

    To make the writing easier, we denote \( X := \ext(D) \) and \( V := V(D) \setminus X \).
    Since \( v \in V \) is not extreme and \( D \) is a tournament, there are \( u,w \in V \) such that \( (u,v),(v,w),(w,u) \in A(D) \).
    Since \( (u,w) \notin A(D) \), we have that a \( (u,w) \)-geodesic must have length at least two. Then, as the path \( (u,v,w) \) exists in \( D \), it is a geodesic.
    We thus conclude that \( v \in I_{\overrightarrow{C3}}( \{ u,w \} ) \).

    Next, we iteratively construct the set \( S \).
    Initially let \( S = \{ u_1,u_2 \} \), with \( u_1,u_2 \) belonging to a common \( C_3 \) (notice that \( |[ S ]_{\overrightarrow{C3}}| \geq 3 \)) and take \( v \in V \setminus [ S ]_{\overrightarrow{C3}} \).
    As we already said there are \( v_1,v_2 \in V \) such that \( (v,v_1),(v_1,v_2),(v_2,v) \in A(D) \).
    We cannot have \( v_1,v_2 \in [S]_{\overrightarrow{C3}} \), because it would result in \( v \in [S]_{\overrightarrow{C3}} \), contradicting its choice.
    If \( v_1,v_2 \) are both not in \( [S]_{\overrightarrow{C3}} \), then we repeat the process and add them to \( S \). Observe that we will have \( v \) in \( [S]_{\overrightarrow{C3}} \), thus obeying the bound.

    Now suppose that for every pair \( v_1,v_2 \) as described above we have \( v_1 \in [S]_{\overrightarrow{C3}} \) and \( v_2 \notin [S]_{\overrightarrow{C3}} \), without loss of generality.
    Since \( v_1 \in [S]_{\overrightarrow{C3}} \) there are \( v_3,v_4 \in [S]_{\overrightarrow{C3}} \) such that \( (v_1,v_3),(v_3,v_4),(v_4,v_1) \in A(D) \).
    If we had \( (v_2,v_4) \in A(D) \), we would also have the directed \( C_3 \) with vertex set \( \{ v_1,v_2,v_4 \} \), contradicting our assumption.
    Thus, we must have \( (v_4,v_2) \in A(D) \).
    We can use an analogous argument to show that we must also have \( (v,v_3) \in A(D) \).
    This leads us to a contradiction: the arc \( (v,v_4) \) would give us the directed \( C_3 \) with vertex set \( \{ v,v_4,v_2 \} \), and the arc \( (v_4,v) \) would give us the directed \( C_3 \) with vertex set \( \{ v,v_3,v_4 \} \).
    Therefore, this situation cannot happen, which means that we always have \( v_1,v_2 \) in one of the two cases presented in the previous paragraph.

    So, we always add two vertices at the same time to \( S \), which in turn increases the cardinality of \( [S]_{\overrightarrow{C3}} \) by at least three.
    In the end, we obtain a set \( S \) such that \( [S]_{\overrightarrow{C3}} = V \) and \( |S| \leq \frac{2}{3}(n(D) - |X| ) \).
    With that in hand, we deduce that \( \ohn (D) \leq |X| + \frac{2}{3}(n(D) - |X|) \), as $S\cup X$ is a hull set of $D$.

    For showing a tight example, we construct a tournament \( D \) such that \( \ohn (D) = |X| + \frac{2}{3}(n(D)-|X|) \).
    See Figure~\ref{fig:proposition.tour} for an illustration of the following construction.
    To ease our arguments we can take a tournament without extreme vertices.
    Let \( \overrightarrow{K_5} \) be a transitive orientation of \( K_5 \) such that \( V(\overrightarrow{K_5}) = \{ 1,2,3,4,5 \} \) and \( A(\overrightarrow{K_5}) = \{ (i,j) \mid i,j \in V(\overrightarrow{K_5}) \textrm{ and } i<j \} \), and let \( \overrightarrow{C_3} \) be a directed \( C_3 \) with vertex set \( \{ u,v,w \} \).
    Our tournament will be \( D = \overrightarrow{K_5} \circ \overrightarrow{C_3} \).

    Take \( (i,u),(j,v) \in V(D) \) such that \( i<j \), then \( ((i,u),(j,v)) \in A(D) \).
    Define \( D_i \), for every \( i \in [5] \), as the copy of \( \overrightarrow{C_3} \) in \( D \) corresponding to the vertex \( i \) of \( \overrightarrow{K_5} \).
    The existence of a \( ((j,v),(i,u)) \)-path implies that there are \( (i',u'),(j',v') \in V(D) \) such that \( i'<j' \) and \( ((j',v'),(i',u')) \in A(D) \), thus contradicting the definition of \( \overrightarrow{K_5} \).
    Moreover, that eliminates the possibility of an \( ((i,u),(i,v)) \)-path that is not contained in \( D_i \).
    From this we conclude that for every \( S \subseteq V(D) \) we have \( I(S) = \bigcup_{i=1}^5 I(S \cap V(D_i)) \) and \( I(S \cap V(D_i)) \subseteq V(D_i) \) for every \( i \in [5] \).
    Therefore, \( [S] = V(D) \) if and only if \( [S \cap V(D_i)] = V(D_i) \) for every \( i \in [5] \), which means that \( \ohn (D) = \sum_{i=1}^5 \ohn (D_i) = 5 \ohn (\overrightarrow{C_3}) \).

    Since \( V(\overrightarrow{C_3}) \geq 2 \) we need at least two vertices to form a hull set of \( \overrightarrow{C_3} \).
    Defining \( A(\overrightarrow{C_3}) = \{ (u,v),(v,w),(w,u) \} \) it is easy to see that \( \ohn (D_2) = 2 \).
    We then have \( \ohn (D) = 10 = \frac{2}{3} 15 = \frac{2}{3} n(D) \).
\end{proof}

One may observe that the tight example in Lemma~\ref{proposition.tour} can be easily generalized to have an arbitrarily large number of vertices, by replacing the transitive orientation of a $K_5$ with one of a $K_n$ for any positive integer $n$.

\begin{figure}[!htb]
    \begin{center}
        \begin{tikzpicture}
            %vértices
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=a3] at (-3,3.08) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=a2] at (-4.62,1.90) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=a4] at (-1.38,1.90) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=a1] at (-4.02,0) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=a5] at (-1.98,0) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=d2] at (3,3.55) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=b2] at (2.6,2.85) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=e2] at (3.4,2.85) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=d3] at (4.62,2.37) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=b3] at (4.22,1.67) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=e3] at (5.02,1.67) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=d4] at (1.38,2.37) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=b4] at (0.98,1.67) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=e4] at (1.78,1.67) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=d5] at (4.02,0.47) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=b5] at (3.62,-0.23) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=e5] at (4.42,-0.23) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=d1] at (1.98,0.47) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=b1] at (1.58,-0.23) {};
            \node[circle,fill=black,inner sep=0pt,minimum size=0.2cm, name=e1] at (2.38,-0.23) {};
            \draw (3,3.08) node [thick, minimum size=1.5cm, draw, circle, name=c3] {};
            \draw (1.38,1.90) node [thick, minimum size=1.5cm, draw, circle, name=c2] {};
            \draw (4.62,1.90) node [thick, minimum size=1.5cm, draw, circle, name=c4] {};
            \draw (1.98,0) node [thick, minimum size=1.5cm, draw, circle, name=c1] {};
            \draw (4.02,0) node [thick, minimum size=1.5cm, draw, circle, name=c5] {};
            %arcos
            \draw[black, thick, ->, >=stealth] (a1) -- (a2);
            \draw[black, thick, ->, >=stealth] (a1) -- (a3);
            \draw[black, thick, ->, >=stealth] (a1) -- (a4);
            \draw[black, thick, ->, >=stealth] (a1) -- (a5);
            \draw[black, thick, ->, >=stealth] (a2) -- (a3);
            \draw[black, thick, ->, >=stealth] (a2) -- (a4);
            \draw[black, thick, ->, >=stealth] (a2) -- (a5);
            \draw[black, thick, ->, >=stealth] (a3) -- (a4);
            \draw[black, thick, ->, >=stealth] (a3) -- (a5);
            \draw[black, thick, ->, >=stealth] (a4) -- (a5);
            \draw[black, thick, ->, >=stealth] (c1) -- (c2);
            \draw[black, thick, ->, >=stealth] (c1) -- (c3);
            \draw[black, thick, ->, >=stealth] (c1) -- (c4);
            \draw[black, thick, ->, >=stealth] (c1) -- (c5);
            \draw[black, thick, ->, >=stealth] (c2) -- (c3);
            \draw[black, thick, ->, >=stealth] (c2) -- (c4);
            \draw[black, thick, ->, >=stealth] (c2) -- (c5);
            \draw[black, thick, ->, >=stealth] (c3) -- (c4);
            \draw[black, thick, ->, >=stealth] (c3) -- (c5);
            \draw[black, thick, ->, >=stealth] (c4) -- (c5);
            \draw[black, thick, ->, >=stealth] (b1) -- (d1);
            \draw[black, thick, ->, >=stealth] (d1) -- (e1);
            \draw[black, thick, ->, >=stealth] (e1) -- (b1);
            \draw[black, thick, ->, >=stealth] (b2) -- (d2);
            \draw[black, thick, ->, >=stealth] (d2) -- (e2);
            \draw[black, thick, ->, >=stealth] (e2) -- (b2);
            \draw[black, thick, ->, >=stealth] (b3) -- (d3);
            \draw[black, thick, ->, >=stealth] (d3) -- (e3);
            \draw[black, thick, ->, >=stealth] (e3) -- (b3);
            \draw[black, thick, ->, >=stealth] (b4) -- (d4);
            \draw[black, thick, ->, >=stealth] (d4) -- (e4);
            \draw[black, thick, ->, >=stealth] (e4) -- (b4);
            \draw[black, thick, ->, >=stealth] (b5) -- (d5);
            \draw[black, thick, ->, >=stealth] (d5) -- (e5);
            \draw[black, thick, ->, >=stealth] (e5) -- (b5);
            \draw[black, thick, ->] (-0.7,1.54) -- (0.2,1.54);
        \end{tikzpicture}
    \end{center}
    \caption{Tight example to Lemma~\ref{proposition.tour}.}
    \label{fig:proposition.tour}
\end{figure}


Now we return to oriented split graphs.
Since in Lemma \ref{proposition.tour} we use only paths of length at most two, we can still find a subset of vertices \( C' \) in the clique $C$ such that $[C' \cup \ext(D[C])] \supseteq C$ and $|C'| \leq \frac{2}{3}(|C \setminus \ext(D[C])|)$.
By Lemma \ref{lemma.non-extremeinS}, we know that $S \setminus \ext(D) \subseteq I(C)$, from where we may deduce the following:

\begin{thm}
    Let $D=(S \cup C,A)$ be an oriented split graph such that $S$ is maximal and $|C| \geq 2$.
    Then, $\ohn (D) \leq |\ext(D) \cap S| + |\ext(D[C])| + \frac{2}{3}|C \setminus \ext(D[C])|$.
\end{thm}
\begin{proof}
    This is a direct consequence of Lemma~\ref{lemma.non-extremeinS} and Lemma~\ref{proposition.tour}.
\end{proof}

==> sec4-npcubes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\NP-completeness for oriented bipartite graphs}
\label{section.bip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we prove that, given a directed bipartite graph $D$ and a positive integer $k$, determining whether $\ohn(D)\leq k$ or whether $\ogn(D)\leq k$ are both \NP-complete problems. Firstly, we study the hull number of a subclass of bipartite graphs called partial cubes.

\subsection{Hull number}

In the undirected case, it was proven that determining the hull number of a graph is an \NP-hard problem, even for partial cubes~\cite{CIPCTHN}, a subclass of bipartite graphs.
Recall that if arcs in both ways were allowed, then this result would imply the \NP-hardness on the oriented case.
As we consider only oriented graphs, we first prove that replacing each edge with a directed $C_4$ has roughly the same effect in the class of bipartite graphs.
%The above result led us to believe that this problem is also difficult for oriented bipartite graphs.
%Our first idea was to try and relate each bipartite graph with an oriented bipartite graph of same hull number.
%We thought that only directing each edge was not enough because we wanted to preserve the paths, so we came up with something else.

Given a (non-oriented) bipartite graph \( G \) with vertex set \( V(G) = \{ v_1, \ldots ,v_n \} \), let \( G_{\oracf} \) be the oriented bipartite graph such that:
\( V(G_{\oracf}) = V(G) \cup \{ v_{i,j},v_{j,i} \mid v_iv_j \in E(G) \} \) and \( A(G_{\oracf}) = \{ (v_i,v_{i,j}),(v_{i,j},v_j),(v_j,v_{j,i}),(v_{j,i},v_i) \mid v_iv_j \in E(G) \} \).

% Given that \( V(G) = \{ v_1, \ldots ,v_n \} \), we start with \( V(G_{\oracf}) = V(G) \) and \( A(G_{\oracf}) = \emptyset \).
% For each pair of adjacent vertices \( v_i \) and \( v_j \) we add the vertices \( v_{i,j} \) and \( v_{j,i} \) to \( V(G_{\oracf}) \) and the arcs \( (v_i,v_{i,j}),(v_{i,j},v_j),(v_j,v_{j,i}),(v_{j,i},v_i) \) to \( A(G_{\oracf}) \).
% We then have 
Thus, we replaced each edge with a directed \( C_4 \).

The first important detail about this procedure is that it ``doubled'' the length of each path in \( G \).
In other words, if we have a path \( P =~v_{i_0}, v_{i_1}, \ldots ,v_{i_k}\) in \( G \) we also have the directed paths:
$P_1 = (v_{i_0}, v_{i_0,i_1}, v_{i_1}, \ldots ,v_{i_{k-1},i_k}, v_{i_k})$ and
$P_2 = (v_{i_k}, v_{i_k,i_{k-1}}, v_{i_{k-1}}, \ldots ,v_{i_1,i_0},v_{i_0}) $ in \( G_{\oracf} \).

Moreover, having \( P_1 \) (resp. \( P_2 \)) in \( G_{\oracf} \) implies the existence of the paths \(P_2\) (resp. \(P_1\)) in \( G_{\oracf} \) and $P$ in  $G$.
Therefore we say that these three are \textit{corresponding paths}.

Notice that for each \( v_iv_j \)-path of length \( d \) in \( G \) we have corresponding \( (v_i,v_j) \)-path and \( (v_j,v_i) \)-path in \( G_{\oracf} \), both of length \( 2d \).
% Thus, \( 2d_G(v_i,v_j) \geq d_{G_{\oracf}}(v_i,v_j) \) and \( 2d_G(v_i,v_j) \geq d_{G_{\oracf}}(v_j,v_i) \) for all \( v_i,v_j \in V(G) \).
% With analogous arguments we obtain \( 2d_G(v_i,v_j) \leq d_{G_{\oracf}}(v_i,v_j) \) and \( 2d_G(v_i,v_j) \leq d_{G_{\oracf}}(v_j,v_i) \) for all \( v_i,v_j \in V(G) \),
Which means that \( 2d_G(v_i,v_j) = d_{G_{\oracf}}(v_i,v_j) = d_{G_{\oracf}}(v_j,v_i) \) for all \( v_i,v_j \in V(G) \).
Consequently, the corresponding paths of a geodesic in \( G \) are also geodesics in \( G_{\oracf} \).

The first result about this transformation does not yet require the graph to be bipartite.

\begin{lem}
    Given a graph \( G \), any of its hull sets is also a hull set of \( G_{\oracf} \).
    Consequently, \( \ohn (G_{\oracf}) \leq \hn (G) \).
\end{lem}

\begin{proof}
    Take a hull set \( S \) of \( G \).
    Since \( S \subseteq V(G) \), every geodesic considered in order to obtain \( I_{G_{\oracf}}[S] \) has a corresponding geodesic in \( G \), and the same is valid for \( I_G[S] \).
    We then have that \( I_{G} [S] = I_{G_{\oracf}} [S] \cap V(G) \).
    Thus, since there are vertices \( v_{i,j} \) in \( I_{G_{\oracf}} [S] \) we can state that \( I_{G}^n [S] \subseteq I_{G_{\oracf}}^n [S] \cap V(G) \) for every \( n \geq 2 \).
    We know that \( [S]_G \subseteq I_{G_{\oracf}}^n [S] \) for some natural \( n \) and that every \( v_{i,j} \) lies in the \( (v_i,v_j) \)-geodesic.
    Therefore, \( I_{G_{\oracf}}^{n+1} [S] \supseteq V(G_{\oracf}) \).
\end{proof}

Next we show the ``converse'' of the above statement: from any hull set of \( G_{\oracf} \) we can obtain a hull set of \( G \) with at most the same cardinality.
However, this fact is only valid for bipartite graphs.

\begin{prop}
    Let \( G \) be a connected bipartite graph and \( S \) a hull set of \( G_{\oracf} \).
    Then, there exists a hull set \( S'\) of \( G \) such that \( |S'| \leq |S| \).
    Therefore, \( \hn (G) \leq \ohn (G_{\oracf}) \).
\end{prop}

\begin{proof}
    Let \( S \) be a hull set of \( G_{\oracf} \).
    We are going to construct another hull set \( S' \) of \( G_{\oracf} \) such that \( |S'| \leq |S| \) and \( S' \subseteq V(G) \).
    Because of the corresponding paths, we deduce that \( S' \) is a hull set of \( G \) and that the proposition holds.


    If \( S \subseteq V(G) \), then take \( S' = S \).
    Otherwise, denote \( S_0 := S \).
    We inductively construct \( S_d \) from \( S_{d-1} \), for \( d > 0 \), by replacing a vertex in \( S_{d-1} \setminus V(G) \) with one in \( V(G) \), preserving the hull set property.

    Let \( v_{i,j} \in S_{d-1} \setminus V(G) \).
    If there is a \( w \in S_{d-1} \setminus \{ v_{i,j} \} \) with some \( (v_{i,j},w) \)-geodesic \( \overrightarrow{P} = (v_{i,j},v_j,v_{j,i},v_i, \ldots ,w) \), notice that there is a \( (v_j,w) \)-geodesic containing \( v_i \) in \( G \).
    Defining \( S_d := (S_{d-1} \setminus \{ v_{i,j} \} ) \cup \{ v_j \} \) gives us \( v_i,v_j \in I[S] \), which implies \( v_{i,j} \in I^2[S] \).
    Thus \( S_{d-1} \subseteq I^2[S_d] \) and, consequently, \( V(G_{\oracf} ) \subseteq [S_{d-1}] \subseteq [S_d] \).
    If we have a \( (w,v_{i,j}) \)-geodesic \( ( w, \ldots ,v_j,v_{j,i},v_i,v_{i,j} ) \), we analogously take \( S_d = (S_{d-1} \setminus \{ v_{i,j} \}) \cup \{ v_i \} \).

    In case such a vertex does not exist in \( S_{d-1} \), then for every \( w \in S_{d-1} \setminus \{ v_{i,j} \} \) the \( (v_{i,j},w) \)-geodesics do not contain \( v_i \) and the \( (w,v_{i,j}) \)-geodesics do not contain \( v_j \).
    Take a vertex \( w \in S_{d-1} \setminus \{ v_{i,j} \} \) and a directed cycle \( C = G_{\oracf} [ \{ v_k,v_{k,l},v_l,v_{l,k} \} ] \) such that \( w \in V(C) \).
    Let \( P_1 \) and \( P_2 \) respectively be a \( (v_{i,j},w) \)-geodesic and a \( (w,v_{i,j}) \)-geodesic.
    In case \( V(P_1) \cap V(P_2) \setminus \{ v_{i,j},w \} \neq \emptyset \), then let \( w' \) belong to this intersection so that the value of \( \min(v_{i,j},w') := \min \{ d(w',v_{i,j}),\) \( d(v_{i,j},w') \} \) is as small as possible.
    If there are \( r,s \) such that \( w' = v_{r,s} \) then we must also have \( v_r \in V(P_1) \) and \( v_s \in V(P_2) \).
    Notice that the \( (v_{i,j},v_r) \)-path contained in \( P_1 \) and the \( (v_s,v_{i,j}) \)-path contained in \( P_2 \) are both geodesics, from where we get \( d(v_{i,j},v_r) = d(v_{i,j},w') - 1 \) and \( d(v_s,v_{i,j}) = d(w',v_{i,j}) - 1 \).
    Thus we have that \( \min (v_{i,j},v_r) \) or \( \min (v_{i,j},v_s) \) is smaller than \( \min (v_{i,j},w') \), contradicting the choice of \( w' \).
    THen we must have \( w' \in V(G) \).

    Observe that the \( (v_j,w') \)-geodesic \( P_1' \) contained in \( P_1 \) has an even number of arcs, \( q_1 \) of the form \( (v_r,v_{r,s}) \) and \( q_1 \) of the form \( (v_{r,s},v_s) \).
    The analogous is true for the \( (w',v_i) \)-geodesic \( P_2' \) contained in \( P_2 \), with length \( 2q_2 \).
    Now, take the \( (w',v_j) \)-path \( P \) such that \( V(P) = (V(P_1') \cap V(G) ) \cup \{ v_{s,r} \mid v_{r,s} \in V(P_1') \} \) and \( A(P) = \{ (v_s,v_{s,r}),(v_{s,r},v_r) \mid (v_r,v_{r,s}),(v_{r,s},v_s) \in A(P_1') \} \).
    Notice that we can extend \( P \) to obtain a \( (w',v_i) \)-path of length \( 2q_1 +2 \) containing \( v_j \), which is not a geodesic due to the case we are working on.
    Thus \( 2q_1+2 > 2q_2 \Rightarrow q_1 \geq q_2 \); analogously \( q_2 \geq q_1 \), giving us \( q_1 = q_2 \).
    We then have that \( P_1' \), \( P_2' \) and the arcs \( (v_i,v_{i,j}),(v_{i,j},v_j) \) together form a directed cycle of length \( 2q_1 + 2q_2 +2 = 2(2q_1 + 1) \).
    In \( G \) there is a corresponding undirected cycle with length \( 2q_1 + 1 \), contradicting the fact that \( G \) is bipartite.
    Since the existence of \( w' \) always results in a contradiction we must have \( V(P_1) \cap V(P_2) = \{ v_{i,j},w \} \).

    By the analysis made in the previous paragraph we cannot have \( w \in \{ v_k,v_l \} \).
    Thus assume without loss of generality that \( w = v_{k,l} \).
    Remember that we are working on the case in which there is no \( (w,v_{i,j}) \)-geodesic and no \( (v_{i,j},w) \)-geodesic containing both \( v_k,v_l \).
    Next we show that we can define \( S_d := ( S_{d-1} \setminus \{ v_{i,j},w \} ) \cup \{ v_i,v_k \} \).

    Let us analyse some \( (v_i,v_k) \)-geodesic \( P_3 \), which uses neither \( v_j \) nor \( v_l \) and has even length \( A(P_3) =: 2p \).
    Let \( P_1'' \) be the \( (v_j,v_k) \)-geodesic contained in \( P_1 \), which also has even length; notice that \( \big| |A(P_3)| - |A(P_1'')| \big| \) must be even.
    If \( |A(P_3)| = |A(P_1'')| \) we would have a directed cycle of length \( 4p + 2 \), which has a corresponding cycle in \( G \) with odd length.
    If \( |A(P_3)| \leq |A(P_1'')| - 2 \) then we could take a path \( P_3' = (v_{i,j},v_j,v_{j,i},v_i, \ldots ,v_k,v_{k,l}) \) containing \( P_3 \) with length \( |A(P_3')| = |A(P_3)| + 4 \leq |A(P_1'')| + 2 = |A(P_1)| \).
    Consequently it would be a \( (v_{i,j},v_{k,l}) \)-geodesic containing both \( v_i \) and \( v_j \), thus contradicting the hypothesis for this case.
    Therefore \( |A(P_3)| \geq |A(P_1'')| + 2 \).
    The argument is analogous for the \( (v_j,v_l) \)-geodesics not containing \( v_i,v_k \).
    Thus the \( (v_i,v_k) \)-path \( P_1' \) with \( V(P_1') = V(P_1'') \cup \{ v_i,v_{i,j} \} \) and \( A(P_1') = A(P_1'') \cup \{ (v_i,v_{i,j}),(v_{i,j},v_j) \} \) is a geodesic.
    Defining the \( (v_k,v_i) \)-path \( P_2' \) analogously we conclude that it is also a geodesic.
    We then have that denoting \( S_d := (S_{d-1} \setminus \{ v_{i,j},v_{k,l} \} ) \cup \{ v_i,v_k \} \) gives us \( v_{i,j},v_{k,l} \in V(P_1') \cup V(P_2') \subset I[S_d] \), which means that \( S_{d-1} \subset I[S_d] \) and consequently \( V(D) \subseteq [S_{d-1}] \subseteq [S_d] \).

    Following these steps inductively we obtain a hull set \( S' \subset V(G) \) of \( G_{\oracf} \).
    Notice that there might be \( v_{i,j},v_{k,l} \in S_d \) with \( \{ i,j \} \cap \{ k,l \} \neq \emptyset \) and that they were both exchanged for the same vertex of \( V(G) \).
    Now we only have left to prove that \( S' \) is also a hull set of \( G \).
    We show by induction on \( k \) that \( I_G^k[S'] = I_{G_{\oracf}}^k [S'] \cap V(G) \).

    Since \( S' \subset V(G) \), for all pairs of vertices \( v_i,v_j \in S' \) every \( (v_i,v_j) \)-geodesic has its corresponding \( v_iv_j \)-geodesic in \( G \).
    Thus it is easy to see that for \( k = 1 \) the claim follows.
    Now assume that it is true for \( k-1 \).
    Seen as \( I_G^{k-1}[S'] = I_{G_{\oracf}}^{k-1}[S'] \cap V(G) \), by the same argument used above it follows that \( I_G^k[S'] = I[ I_{G_{\oracf}}^{k-1}[S'] \cap V(G) ] \cap V(G) \subseteq I_{G_{\oracf}}^k[S'] \cap V(G) \).
    Next we show that \( I_{G_{\oracf}}^k[S'] \cap V(G) \subseteq I_G^k[S'] \).

    Taking \( w \in \left( I_{G_{\oracf}}^k[S'] \cap V(G) \right) \setminus I_{G_{\oracf}}^{k-1}[S'] \), we know that there are \( w_1,w_2 \in I_{G_{\oracf}}^{k-1}[S'] \) such that \( w \) lies in some \( (w_1,w_2) \)-geodesic.
    If both \( w_1,w_2 \) are vertices of \( G \) then we clearly have \( w \in I_G^k[S'] \).
    Suppose that there are distinct \( i,j \in \{ 1, \ldots ,n(G) \} \) such that \( w_1 = v_{i,j} \).
    Since \( S' \subset V(G) \) let \( k' \in [k-1] \) be such that \( w_1 \notin I_{G_{\oracf}}^{k'-1}[S'] \) and \( w_1 \in I_{G_{\oracf}}^{k'}[S'] \).
    Thus there are \( w_3,w_4 \in I_{G_{\oracf}}^{k'-1}[S'] \) such that \( w_1 \) is interior to some \( (w_3,w_4) \)-geodesic.
    We know that both indegree and outdegree of \( w_1 \) are equal to one, which means that \( v_i,v_j \in I_{G_{\oracf}}^{k'}[S'] \).
    Define \( w_1' \) as \( w_1 \) if this belongs to \( V(G) \), and as \( v_j \) otherwise.
    Similarly define \( w_2' \).
    In any event we have a \( (w_1',w_2') \)-geodesic contained in the \( (w_1,w_2) \)-geodesic mentioned before.
    It is easy to see now that \( w \in I_G^k[S'] \).
    This concludes our demonstration.
\end{proof}

To emphasize the necessite of \( D \) being bipartite in the previous proposition, we show a non-bipartite graph that violates the stated inequality.
Let \( G = C_3 \) with vertices \( v_1,v_2,v_3 \).
Since it is a complete graph, all its vertices are simplicials and therefore \( \hn (G) = 3 \).
Now considering \( G_{\oracf} \), notice that \( (v_{1,2},v_2,v_{2,3},v_3) \) and \( (v_3,v_{3,1},v_1,v_{1,2}) \) are both geodesics, thus \( v_1,v_2,v_3 \in I[ \{ v_{1,2},v_3 \} ] \).
We then conclude that \( I^2[ \{ v_{1,2},v_3 \} ] = V(G_{\oracf}) \), hence \( \ohn (G_{\oracf}) = 2 \).

\begin{thm}
    \label{thm.npcbip}
    If $G$ is a bipartite graph, then $\hn (G) = \ohn (G_{\oracf})$.
\end{thm}

It was proven in~\cite{OTHNOSGC} that determining whether \( \hn (G) \leq k \) is \NP-complete for a bipartite graph \( G \).
Thus, one can combine this result with Corollary~\ref{thm.npcbip} to deduce that, given an oriented bipartite graph $D$ and a positive integer $k$, deciding whether $\ohn (D) \leq k$ is an \NP-complete problem.
However, one can observe that such reduction can also be applied to partial cubes, a subclass of bipartite graphs, which we define in the sequel.
%Now that we have two comparable parameters and one of them is difficult, it is only natural that the other will be too.

%Inspired by this result we thought if the hull number problem was also hard for a subclass of oriented bipartite graphs, to make a stronger statement.
%Our first idea would be to use the \( G_{\oracf} \), but for that this problem would have to be difficult in the non-oriented case as well.
%We were fortunate to find a desired result.

The \textit{hypercube graph of dimension n}, \( Q_n \), is a (undirected) graph such that its vertex set is \( V(Q_n) = \{ 0,1 \}^n \).
We express each vertex as \( v = (v^1, \ldots ,v^n) \), where \( v^i \in \{ 0,1 \} \) for every \( i \in \{ 1, \ldots ,n \} \).
The edge set of $Q_n$ is \( E(Q_n) = \{ uv \mid \) there is exactly one \( i \in \{ 1, \ldots ,n \} \) such that \( u^i \neq v^i \} \).
A \textit{partial cube} graph \( G \) is an isometric subgraph of some \( Q_n \), meaning that \( d_G(u,v) = d_{Q_n}(u,v) \) for every \( u,v \in V(G) \).
Moreover, since hypercubes are connected then the distance between each pair of vertices is positive and finite, hence partial cubes are also connected.

Computing the hull number of partial cubes is also an \NP-hard problem~\cite{CIPCTHN}.
Thus due to Theorem~\ref{thm.npcbip}, we only have to show that given a partial cube graph \( G \), \( G_{\oracf} \) is an oriented partial cube.

\begin{prop}
    If $G$ is a partial cube, then $G_{\oracf}$ is an oriented partial cube.
\end{prop}

\begin{proof}
    Let \( G \) be a partial cube with \( V(G) = \{ v_1, \ldots ,v_l \} \).
    If \( k \) is the smallest positive integer such that \( G \subseteq Q_k \), each vertex of \( G \) can be considered as an element of \( \{ 0,1 \}^k \).
    Thus let \( H \subseteq Q_{2k} \) be a graph initially with \( V(H) = \{ u_1, \ldots ,u_l \} \subseteq \{ 0,1 \}^{2k} \) and, for each \( u_i = (u_i^1,u_i^2, \ldots ,u_i^{2k}) \) and \( v_i = (v_i^1,v_i^2, \ldots ,v_i^k) \), \( u_i^{2j-1} = u_i^{2j} = v_i^j \) for every \( j \in \{ 1, \ldots ,k \} \).
    Notice that each two vertices \( u_i \) and \( u_j \) differ in a positive even number of entries.

    Take two distinct vertices \( u_i,u_j \in V(H) \) such that there is only one \( m \in \{ 1, \ldots ,k \} \) so that \( u_i^{2m-1} = u_{i}^{2m} \neq u_j^{2m-1} = u_j^{2m} \) (notice that \( v_i,v_j \) are adjacent in \( G \)).
    For each such pair add the vertices \( u_{i,j} = (u_i^1, \ldots ,u_i^{2m-1},u_j^{2m},u_i^{2m+1}, \ldots ,\) \( u_i^{2k}) \) and \( u_{j,i} = (u_j^1, \ldots ,u_j^{2m-1},u_i^{2m},u_j^{2m+1}, \ldots ,u_j^{2k}) \) to \( V(H) \), which differ in the \( 2m-1^{\textrm{th}} \) and \( 2m^{\textrm{th}} \) entries.
    Notice also that both \( u_i \) and \( u_j \) differ in exactly one entry from both \( u_{i,j} \) and \( u_{j,i} \).
    Moreover add the edges \( u_iu_{i,j},u_{i,j}u_j,u_ju_{j,i},\) \(u_{j,i}u_i \) to \( E(H) \), which if oriented as \( (u_i,u_{i,j}),(u_{i,j},u_j),(u_j,u_{j,i}),(u_{j,i},u_i) \) result in \( G_{\oracf} \).

    Next we analyse each kind of pair of vertices of \( H \).
    If our pair is \( u_p,u_q \) we already know that they have at least two distinct entries.
    If it is \( u_p,u_{q,r} \) with \( p \in \{ q,r \} \) we also know that they have all but one entries in common.
    Now take \( p,q,r \in \{ 1, \ldots ,l \} \) such that \( u_{p,q} \in V(H) \) and \( r \notin \{ p,q \} \).
    Define \( m \colon \{ 1, \ldots ,l \}^2 \to \{ 0,1, \ldots ,k \} \) as \( m(i,j)=0 \) if either \( i=j \) or if \( u_i,u_j \) are not adjacent, and as the only \( m \in \{ 1, \ldots ,k \} \) such that \( u_i^{2m} \neq u_j^{2m} \) for every other pair \( (i,j) \).
    Since \( r \notin \{ p,q \} \), there must be \( m \in \{ 1, \ldots ,k \} \setminus \{ m(p,q) \} \) such that \( u_r^{2m-1} = u_r^{2m} \neq u_p^{2m-1} = u_p^{2m} \).
    We know that the \( 2m-1^{\textrm{th}} \) and the \( 2m^{\textrm{th}} \) entries of \( u_p \) and \( u_{p,q} \) are equal, thus \( u_r \) and \( u_{p,q} \) have at least two distinct entries.

    The last case is a pair \( u_{p,q},u_{r,s} \).
    If \( d_G(v_i,v_j) = 1 \) for every \( i \in \{ p,q \} \) and every \( j \in \{ r,s \} \), since \( v_p \) and \( v_q \) are adjacent in \( G \) by the existence of \( u_{p,q} \) we would have triangles in \( G \), which is not possible since it is bipartite.
    Thus there are \( i \in \{ p,q \} \) and \( j \in \{ r,s \} \) such that \( d_G(v_i,v_j) \geq 2 \), which means that we have \( m_1, \ldots ,m_t \in \{ 1, \ldots ,k \} \) such that \( v_i^m \neq v_j^m \) for every \( m \in \{ m_1, \ldots ,m_t \} \) and \( t = d_G(v_i,v_j) \).
    Suppose that there is some \( m \) in the previous set which is not in \( \{ m(p,q),m(r,s) \} \), then \( u_p^{2m-1} = u_p^{2m} = u_q^{2m-1} = u_q^{2m} \neq u_r^{2m-1} = u_r^{2m} = u_s^{2m-1} = u_s^{2m} \).
    Consequently, \( u_{p,q} \) and \( u_{r,s} \) have at least two distinct entries.
    Else we must have \( t=2 \), \( m_1 = m(p,q) \) and \( m_2 = m(r,s) \), without loss of generality.
    Notice that \( u_r^{2m_1-1} = u_r^{2m_1} = u_s^{2m_1-1} = u_s^{2m_1} \) and \( u_p^{2m_1-1} = u_p^{2m_1} \neq u_q^{2m_1-1} = u_q^{2m_1} \), which means that either the \( 2m_1-1^{\textrm{th}} \) or the \( 2m_1^{\textrm{th}} \) positions of \( u_{r,s} \) and \( u_{p,q} \) are different.
    The same can be said about the \( 2m_2-1^{\textrm{th}} \) and \( 2m_2^{\textrm{th}} \) positions, thus \( u_{p,q} \) and \( u_{r,s} \) have at least two distinct entries.
    Therefore, if we combine the results of these last two paragraphs with the construction of \( H \), we conclude that two vertices of \( H \) are adjacent if and only if they have only one distinct entry.

    That being said, all that is left to prove is that \( d_H(u,v) = d_{Q_{2k}}(u,v) \) for every \( u,v \in V(H) \).
    First consider \( u_i \) and \( u_j \).
    If \( v_i \) and \( v_j \) have \( p \) different entries, than their corresponding vertices in \( H \) differ in \( 2p \) entries implying that \( d_{Q_{2k}}(u_i,u_j) = 2p \).
    Since \( G \) is a partial cube we know that \( d_G(v_i,v_j) = d_{Q_k}(v_i,v_j) = p \), thus there is a \( v_iv_j \)-path with length \( p \) in \( G \).
    Due to the construction of \( H \), we also have in it a \( u_iu_j \)-path of length \( 2p \).
    Now suppose that there is a \( u_iu_j \)-path in \( H \) with length \( q < 2p \).
    Seen as the neighbors in \( H \) have exactly one distinct entry, then the endvertices of this path differ in at most \( q \) entries, which is a contradiction.
    Thus \( d_H(u_i,u_j) = 2p \).

    Next we analyze the distance between \( u_{i,j} \) and \( u_{r,s} \).
    Let \( \{ u,u' \} = \{ u_i,u_j \} \) and \( \{ v,v' \} = \{ u_r,u_s \} \) be such that \( u \) and \( v \) are as close as possible.
    It is straightforward that \( d_H(u_{i,j},u_{r,s}) = 2 + d_H(u,v) = 2(p+1) \), where \( 2p \) is the number of distinct entries of \( u \) and \( v \).
    Since we change one entry from \( u \) to \( u_{i,j} \) and one from \( v \) to \( u_{r,s} \) we must have \( 2p+2 \) distinct entries between \( u_{i,j} \) and \( u_{r,s} \), meaning that \( d_{Q_{2k}}(u_{i,j},u_{r,s}) = 2p+2 \).
    This also covers the proof that \( d_H(u_{i,j},u_r) = d_{Q_{2k}}(u_{i,j},u_r) \).
\end{proof}

\begin{cor}
    Given an oriented partial cube \( D \) and a positive integer \( k \), it is \NP-complete to decide whether \( \ohn(D) \leq k \).
\end{cor}

%That ends the hull number problem for this section, we now discuss the geodetic number.

\subsection{Geodetic number}

\newcommand\myprob[3]{%

\vspace{0.3cm}

\par\noindent #1\\

{\bfseries Input}: #2\\

{\bfseries Output}: #3\par

\vspace{0.3cm}

}


Our goal in this section is to prove that the following problem is \NP-complete:

\myprob{\textsc{Oriented Geodetic Number}}{Oriented graph $D$ and a positive integer $k$}{$\ogn(D)\leq k?$}


\begin{thm}\label{teo.npgndag}
    \textsc{Oriented Geodetic Number} is an \NP-complete problem, even if the input oriented graph $D$ has no directed cycle and a bipartite underlying graph.
\end{thm}
\begin{proof}
    Given a subset of vertices $S\subseteq V(D)$, one can compute $(u,v)$-geodesics, for every $u,v\in V(D)$, and decide whether $S$ is a geodetic set in polynomial time similarly to the undirected case~\cite{TGHNIHFCG}.
    Consequently, the problem is in \NP.

    We reduce the well-known \textsc{Set Cover}~\cite{Karp72} problem to \textsc{Oriented Geodetic Number}:

    \myprob{\textsc{Set Cover}}{\( U= \{ 1,2, \ldots ,n \} \), \( \mathcal{F} \subseteq \mathcal{P}(U) \) such that \( \bigcup \mathcal{F} = U \) and a positive integer $k$}{Does there exist \( \mathcal{F}' \subseteq \mathcal{F} \) such that \( \bigcup \mathcal{F}' = U \) and $|\mathcal{F'}|\leq k$?}


    Let $(U= \{ 1,2, \ldots ,n \}, \mathcal{F} = \{F_1,\ldots, F_m\},k)$ be an input to \textsc{Set Cover}.
    We shall construct an oriented graph $D$ such that $(U, \mathcal{F},k)$ is an YES-instance if, and only if, $\ogn(D)\leq k+3$.

    The vertex set of $D$ is composed by two subsets of vertices $X$ and $Y$ union three vertices $u$, $v$ and $w$.
    In $X$ there is one vertex $u_i$ corresponding to $F_i\in\mathcal{F}$, for every $i\in\{1,\ldots, m\}$.
    In $Y$ there is a vertex $v_j$ corresponding to each element $j \in U$.

    %In the arc set of $D$ there is the arc $(u_i,v_j)\in A(D)$ whenever $j \in F_i$, for every $i\in\{1,\ldots, m\}$ and $j\in\{1,\ldots,n\}$.
    %Moreover, $A(D)$ has the arcs $(u,u_i),(u_i,w)$ for every $i \in \{1,\ldots, m\}$, the arcs $(v_j,v)$ for every $j \in \{1,\ldots,n\}$, and finally the arc $(u,v)$.
    
    
    Next we describe the arc set of \( D \).
    For every $i\in\{1,\ldots, m\}$ and $j\in\{1,\ldots,n\}$, whenever $j \in F_i$ we have $(u_i,v_j) \in A(D)$.
    The remaining arcs of $A(D)$ are the following: $(u,u_i),(u_i,w)$ for every $i \in \{1,\ldots, m\}$, $(v_j,v)$ for every $j \in \{1,\ldots,n\}$, and finally $(u,v)$.

    By construction, $D$ is clearly a DAG whose underlying graph is bipartite (with partition \( V(D) = (X \cup \{ v \} ) \cup (Y \cup \{ u,w \} ) \)).
    Figure \ref{fig.scdag} exemplifies $D$ when $U = \{ 1,2,3,4,5 \}$ and $\mathcal{F} = \{ F_1 = \{ 1,2,3,4 \},F_2 = \{ 1,4 \},F_3 = \{ 2,3,5 \} \}$.
    Notice that $u$ is a source and that $v$ and $w$ are sinks, thus they belong to any geodetic set.
    Besides, \( (u,w) \notin A(D) \) and for every \( u_i \in X \) we have the path \( (u,u_i,w) \).
    Since \( (u,v) \in A(D) \) we have \( I[u,v,w] = X \cup \{ u,v,w \} \).
    
    \begin{figure}[!htb]
        \begin{center}
            \begin{tikzpicture}
                %nodes
                \node[black] at (1.5,2.2) {\( y_1 \)};
                \node[black] at (1.5,1.3) {\( y_2 \)};
                \node[black] at (1.5,0.4) {\( y_3 \)};
                \node[black] at (1.5,-0.5) {\( y_4 \)};
                \node[black] at (1.5,-1.4) {\( y_5 \)};
                \node[black] at (1.5,-2.5) {\( Y \)};
                \node[black] at (-1.5,1.75) {\( x_1 \)};
                \node[black] at (-1.5,0.4) {\( x_2 \)};
                \node[black] at (-1.5,-0.95) {\( x_3 \)};
                \node[black] at (-1.5,-2.5) {\( X \)};
                \node[black] at (-3.9,0) {\( u \)};
                \node[black] at (3.9,0) {\( v \)};
                \node[black] at (0.4,-2.5) {\( w \)};
                %ellipses
                \draw[black, thick] (1.5,0.15) ellipse (0.7cm and 2.3cm);
                \draw[black, thick] (-1.5,0.15) ellipse (0.7cm and 2.3cm);
                %vertices
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=1] at (1.5,1.8) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=2] at (1.5,0.9) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=3] at (1.5,0) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=4] at (1.5,-0.9) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=5] at (1.5,-1.8) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=f1] at (-1.5,1.35) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=f2] at (-1.5,0) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=f3] at (-1.5,-1.35) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=u] at (-3.5,0) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=v] at (3.5,0) {};
                \node[circle,fill=black,inner sep=0pt,minimum size=0.3cm, name=w] at (0,-2.5) {};
                %arcs
                \draw[black, thick, ->, >=stealth] (-3.5,0) arc (180:3:3.5);
                %\draw[black, thick, ->, >=stealth] (u) to [out=90,in=90] (v);
                \draw[black, thick, ->, >=stealth] (f1) -- (1);
                \draw[black, thick, ->, >=stealth] (f1) -- (2);
                \draw[black, thick, ->, >=stealth] (f1) -- (3);
                \draw[black, thick, ->, >=stealth] (f1) -- (4);
                \draw[black, thick, ->, >=stealth] (f2) -- (1);
                \draw[black, thick, ->, >=stealth] (f2) -- (4);
                \draw[black, thick, ->, >=stealth] (f3) -- (2);
                \draw[black, thick, ->, >=stealth] (f3) -- (3);
                \draw[black, thick, ->, >=stealth] (f3) -- (5);
                \draw[black, thick, ->, >=stealth] (u) -- (f1);
                \draw[black, thick, ->, >=stealth] (u) -- (f2);
                \draw[black, thick, ->, >=stealth] (u) -- (f3);
                \draw[black, thick, ->, >=stealth] (f1) -- (w);
                \draw[black, thick, ->, >=stealth] (f2) -- (w);
                \draw[black, thick, ->, >=stealth] (f3) -- (w);
                \draw[black, thick, ->, >=stealth] (1) -- (v);
                \draw[black, thick, ->, >=stealth] (2) -- (v);
                \draw[black, thick, ->, >=stealth] (3) -- (v);
                \draw[black, thick, ->, >=stealth] (4) -- (v);
                \draw[black, thick, ->, >=stealth] (5) -- (v);
            \end{tikzpicture}
            \caption{Oriented graph constructed in the proof of Theorem \ref{teo.npgndag}, assuming \( U = \{ 1,2,3,4,5 \} \) and \( \mathcal{F} = \{ F_1 = \{ 1,2,3,4 \},F_2 = \{ 1,4 \},F_3 = \{ 2,3,5 \} \} \).}
            \label{fig.scdag}
        \end{center}
    \end{figure}

    Let $\mathcal{F}' = \{ F_i \mid i \in I\} \subseteq \mathcal{F}$, for some $I\subseteq \{1,\ldots, m\}$ such that $\bigcup_{i\in I} F_{i} = U$ and $|I| \leq k$.
    We then take $ X' = \{ u_i \mid i\in I \} \cup \{ u,v,w \} $, which has cardinality at most \( k+3 \).
    Thus, for every \( v_j \in Y \) there is \( u_i \in X' \) such that \( (u_i,v_j) \in A(D) \), from where we have the geodesic \( (u_i,v_j,v) \).
    Therefore, one can observe that $X'$ is a geodetic set of $D$.

    On the other hand, let $S$ be a geodetic set of $D$ with at most $k+3$ vertices.
    Thus, $\{u,v,w\}\subseteq S$ and at most $k$ vertices of $S$ belong to $X\cup Y$.
    If some $v_j\in S$, one can observe that by replacing $v_j$ with a vertex $u_i$ such that $(u_i,v_j)\in A(D)$, we obtain another geodetic set $S'$ such that $|S'|\leq k+3$.
    Thus, without loss of generality, we assume that $S\setminus\{u,v,w\}\subseteq X$.
    Let $I=\{i\in\{1,\ldots,m\}\mid u_i\in S\}$.
    One can also observe that the family $\mathcal{F'} = \{F_i\in F\mid i\in I\}$ satisfies $\bigcup \mathcal{F'} = U$ and $|\mathcal{F'}| \leq k$.
    \end{proof}

    One may observe that the previous reduction can be done in linear time and the corresponding values of the solutions of the instances differ by 3 units.
    Then, it also implies that \textsc{Oriented Geodetic Number} is \textsl{W}[2]-hard, when parameterized by the value of the solution $k$, and it does not admit a polynomial-time approximation algorithm with ratio $c\cdot \ln n$, unless $\Poly=\NP$, even if the input graph is a DAG having a bipartite underlying graph, as these hardness results are also valid for the \textsc{Set Cover} problem~\cite{RS1997,DF2012}.  
